Personality Anchoring for Social Simulation: Linking Personality, Social Behavior, and Interaction Success with LLM Agents

Social interactions are shaped by the interplay of dispositional traits and situational context, yet systematically investigating how personality configurations between individuals jointly influence social behavior across diverse social contexts remains methodologically challenging. We address this gap by introducing a simulation pipeline adapted from the CHARISMA framework, which employs well-known movie characters and public figures as psychologically grounded agents for multi-LLM social simulation using a method we term personality anchoring. We present a large-scale empirical study examining how dyadic Agreeableness composition influences social interaction outcomes across 1,010 simulated conversations. Our results reveal a monotonic relationship between dyadic Agreeableness composition and shared goal achievement, with Homogeneous-Agreeable pairs achieving success 10 times the rate of Homogeneous-Disagreeable pairs (62% vs. 6%). Behavioral mediation analysis reveals that Agreeableness shapes goal achievement partially through cooperative strategy selection, though it continues to predict outcomes within the same dominant strategy, indicating pathways beyond observable conversational behavior. Robustness analyses confirm high consistency of results across repeated simulations (ICC = 0.89) and stable personality expression across diverse scenarios, validating personality anchoring as a viable operationalization strategy.

==> latex/99-macros.tex <==
\usepackage{hyperref}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{amsmath}
\usepackage{textgreek}
\usepackage[table]{xcolor}
\usepackage{multirow}

\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}

\newcommand{\eg}{{e.g., }}
\newcommand{\ie}{{i.e., }}
\newcommand{\charisma}{{\textbf{CHARISMA}}}

\definecolor{dgrey}{gray}{0.2}
\newcommand{\blue}[1]{\textcolor{RoyalBlue}{#1}}
\newcommand{\grey}[1]{\textcolor{dgrey}{#1}}
\newcommand{\lf}[1]{\textcolor{green}{\textbf{[[LF: #1]]}}} %comments from Lucie
\newcommand{\vs}[1]{\textcolor{blue}{\textbf{[[VS: #1]]}}} %comments from Vahid
\newcommand{\MYhref}[3][blue]{\href{#2}{\color{#1}{#3}}}
\newcommand{\jt}[1]{\textcolor{teal}{\textbf{[[JT: #1]]}}} %comments from Johanne

\usepackage{balance} % For balanced columns on the last page

\newcommand{\mycaption}[1]{\caption{\normalfont{#1}}}
\newcommand{\myparagraph}[1]{\vspace{0.5\baselineskip}\noindent{\textbf{#1}}.~}
